A Survey on Automated Fact-Checking

Fact-checking has become increasingly important due to the speed with which both information and misinformation can spread in the modern media ecosystem. Therefore, researchers have been exploring how fact-checking can be automated, using techniques based on natural language processing, machine learning, knowledge representation, and databases to automatically predict the veracity of claims. In this paper, we survey automated fact-checking stemming from natural language processing, and discuss its connections to related tasks and disciplines. In this process, we present an overview of existing datasets and models, aiming to unify the various definitions given and identify common concepts. Finally, we highlight challenges for future research.

==> tables/ar_poster.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lccccccccccc}
\toprule
Dataset & Input & \#Inputs & Evidence & Verdict & Sources & Lang \\
\midrule
FEVER~\citep{Thorne2018FEVERAL} & State & 185,445  & Text & 3Class & Wiki & En \\
HOVER~\citep{jiang2020hover} & State & 26,171  & Text & 2Class & Wiki & En  \\
% WikiFactCheck~\citep{SatheALPP20} & State & 124,821  & Text & 2Class & Wiki & En  \\
% Symmetric \citep{Schuster2019TowardsDF} & State & 956  & Text & 3 & Wikipedia & En \\
% FM2 \citep{foolme2021} & State & 12,968  & Text & 3 & Wikipedia & En \\
VitaminC~\citep{vitaminc2021} & State & 488,904  & Text & 3Class & Wiki & En \\
TabFact~\citep{Chen2020TabFactAL} & State & 92,283  & Table & 2Class & Wiki & En \\
InfoTabs~\citep{Gupta2020INFOTABSIO} & State & 23,738  & Table & 3Class & Wiki & En \\
Sem-Tab-Fact~\citep{wang2021semeval} & State & 5,715  & Table & 3Class & Wiki & En \\
FEVEROUS~\citep{Aly2021FEVEROUSFE} & State & 87,026  & Text/Table & 3Class & Wiki & En \\
% ANT~\citep{Khouja2020StancePA} & State & 4,547  & \xmark & 3Class & News & Ar \\
% DanFEVER~\citep{NorregaardD21} & State & 6,407  & Text & 3 Classes & Wiki & Da \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of factual verification datasets with artificial inputs. Google denotes Google Relation Extraction Corpora, and WSDM means the WSDM Cup 2017 Triple Scoring challenge.}
\label{tab:artificial}
\vspace{-1em}
\end{table*}

==> tables/de_poster.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lcccccc}
\toprule
Dataset & Type & Input & \#Inputs & Evidence & Verdict & Lang \\
\midrule
CredBank~\citep{MitraG15} & Worthy & Aggregate & 1,049  & Meta & 5 Classes  & En \\
Weibo~\citep{Ma2016DetectingRF} & Worthy & Aggregate & 5,656  & Meta & 2 Classes  & En/Ch  \\
% Weibo20 \citep{zhang2021mining} & Aggregate & 6,362 & 2 & Meta & Weibo & Ch \\
PHEME~\citep{zubiaga2016analysing} & Worthy & Individual & 330  & Text/Meta & 3 Classes  & En/De \\
% RumourEval \citep{Derczynski2017SemEval2017T8} & Worthy & Individual & 325  & Text/Meta & 3 & Twitter & En \\
RumourEval19~\citep{GorrellABDKLZ19} & Worthy & Individual & 446 & Text/Meta & 3 Classes  & En \\
DAST~\citep{Lillie2019JointRS} & Worthy & Individual & 220  & Text/Meta & 3 Classes  & Da \\
Suspicious~\citep{Volkova2017SeparatingFF} & Worthy & Individual & 131,584  & \xmark & 2/5 Classes  & En \\
CheckThat20-T1~\citep{BarrnCedeo2020OverviewOC} & Worthy & Individual & 8,812  & \xmark & Ranking  & En/Ar \\
CheckThat21-T1A~\citep{NakovMEBMSAHHBN21} & Worthy & Individual & 17,282  & \xmark & 2 Classes & Many \\
% FauxBuster \citep{Zhang2018FauxBusterAC} & Worthy & Individual$^{\dagger}$ & 917  & Meta  & 2 & Twitter/Reddit & En \\
% COVIDLIES \citep{Hossain2020COVIDLiesDC} & Worthy & Individual & 6,761 & Misconception & 3 & Twitter & En \\
% \midrule
Debate~\citep{hassan2015detecting} & Worthy & Statement & 1,571  & \xmark & 3 Classes  & En \\
ClaimRank~\citep{Gencheva2017ACA} & Worthy & Statement & 5,415  & \xmark & Ranking  & En \\
CheckThat18-T1~\citep{Atanasova2018OverviewOT} & Worthy & Statement & 16,200  & \xmark & Ranking  & En/Ar \\
% CheckThat19-T1 \citep{CheckThat2019} & Claim & 23,500 & ranking & \xmark & Transcript & En \\
% CheckThat20-T5 \citep{BarrnCedeo2020OverviewOC} & Claim & 64,290 & ranking & \xmark & Transcript & En \\
% CheckThat21-T1B \citep{clef2021} & Claim & 84,290 & ranking & \xmark & Transcript & En \\
\midrule
%\midrule
CitationReason~\citep{redi2019}  & Checkable & Statement & 4,000  & Meta & 13 Classes  & En \\
PolitiTV~\citep{konstantinovskiy2018towards} & Checkable & Statement & 6,304  & \xmark & 7 Classes  & En \\
%SemEval19-TA\citep{Mihaylova2019SemEval2019T8} & Checkable & Question & 2,310 & Meta  & 3 & Forum & En \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of claim detection datasets. Input can be a set of posts (aggregate) or an individual post from social media, or a statement. Evidence include text and metadata. Verdict can be a multi-class label or a rank list.}
% En, De, Ch, Ar, and Da indicate English, German, Chinese, Arabic, and Danish, respectively.}
% \citet{NakovMEBMSAHHBN21} offered datasets in Arabic, Bulgarian, English, and Spanish.}
\label{tab:detection}
\vspace{-1em}
\end{table*}

==> tables/na_poster.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lccccccccccc}
\toprule
Dataset & Input & \#Inputs & Evidence & Verdict & Sources & Lang \\
\midrule

Politifact~\citep{Vlachos2014FactCT}  & State  & 106  & Text/Meta & 5Class & Factcheck & En \\
% NewsTrust \citep{Mukherjee2015LeveragingJI}  & State  & 106 & 5 & Text  & Factcheck & En \\
Emergent~\citep{Ferreira2016EmergentAN} & State & 300  & Text & 3Class & Emergent & En \\
% CreditAssess~\citep{Popat2016CredibilityAO} & State & 5,013 & Text & 2 Classes & Factcheck/Wiki & En \\
PunditFact~\citep{Rashkin2017TruthOV} & State  & 4,361  & \xmark & 2/6Class & Factcheck & En \\
Liar~\citep{Wang2017LiarLP} & State  & 12,836  & Meta & 6Class & Factcheck & En \\
% Liar-Plus \citep{Alhindi2018WhereIY} & State & 12,836 & 6 & Text/Meta & Factcheck & En \\
% CheckThat19-T2 \citep{HasanainSEBN19} & State &  69  & Text & 2 & News & En\\
Snopes~\citep{Hanselowski2019ARA} & State & 6,422  & Text & 3Class & Factcheck & En \\
MultiFC~\citep{Augenstein2019MultiFCAR} & State & 36,534  & Text/Meta & 2-27Class &  Factcheck & En \\
% Climate-FEVER~\citep{diggelmann2020} & State & 1,535 & Text  & 4 Classes & Climate & En \\
SciFact~\citep{Wadden2020FactOF} & State & 1,409  & Text & 3Class & Science & En \\
Health~\citep{kotonya2020explainable} & State & 11,832  & Text & 4Class & Factcheck & En\\

X-Fact~\citep{gupta-srikumar-2021-x} & State & 31,189  & Text & 7Class & Factcheck & Many\\
\midrule
FEVER~\citep{Thorne2018FEVERAL} & State & 185,445  & Text & 3Class & Wiki & En \\
HOVER~\citep{jiang2020hover} & State & 26,171  & Text & 2Class & Wiki & En  \\
% WikiFactCheck~\citep{SatheALPP20} & State & 124,821  & Text & 2Class & Wiki & En  \\
% Symmetric \citep{Schuster2019TowardsDF} & State & 956  & Text & 3 & Wikipedia & En \\
% FM2 \citep{foolme2021} & State & 12,968  & Text & 3 & Wikipedia & En \\
VitaminC~\citep{vitaminc2021} & State & 488,904  & Text & 3Class & Wiki & En \\
TabFact~\citep{Chen2020TabFactAL} & State & 92,283  & Table & 2Class & Wiki & En \\
InfoTabs~\citep{Gupta2020INFOTABSIO} & State & 23,738  & Table & 3Class & Wiki & En \\
Sem-Tab-Fact~\citep{wang2021semeval} & State & 5,715  & Table & 3Class & Wiki & En \\
FEVEROUS~\citep{Aly2021FEVEROUSFE} & State & 87,026  & Text/Table & 3Class & Wiki & En \\
% \midrule
% % SemEval19-TB \citep{Mihaylova2019SemEval2019T8} & Answer & 917  & Meta & 3 & Forum & En \\
% AnswerFact~\citep{Zhang2020AnswerFactFC} & Answer & 60,864 & Text & 5 Classes & Amazon & En \\
% \midrule
% % Hoax \citep{TacchiniBVMA17} & Article & 15,500  & Meta & 2 Classes & Facebook & En \\
% NELA~\citep{HorneKA18} & Article & 136,000  & \xmark & 2 Classes & News & En \\
% BuzzfeedNews \citep{Potthast2018ASI} & Article & 1,627 & Meta & 4 Classes & Facebook & En \\
% BuzzFace~\citep{SantiaW18} & Article & 2,263 & Meta & 4 Classes & Facebook & En \\
% % NELA18 \citep{Nrregaard2019NELAGT2018AL} & Article & 713,000 & 2 & \xmark & News & En \\
% % NELA19 \citep{gruppi2020nela} & Article & 1.12M & 2 & \xmark & News & En \\
% FA-KES~\citep{SalemFEJF19} & Article & 804 & \xmark & 2 Classes & VDC & En \\
% FakeNewsNet \citep{Shu2018FakeNewsNetAD} & Article & 23,196  & Meta & 2 Classes & Factcheck & En \\
% %FakeHealth \citep{DaiSW20} & Article & 2,296  & Meta & 2 Classes & Health & En \\
% FakeCovid~\citep{shahifakecovid} & Article & 5,182  & \xmark & 2 Classes & Factcheck & Many \\
% \midrule
% Fauxtography \citep{Zlatkova2019FactCheckingMF} & State/Image & 1,233  & Meta & 2 & Factcheck/News & En \\
% Fakeddit \citep{Nakamura2020rFakedditAN} & State/Image & 1.06M  & Meta & 2,3,6 & Reddit & En \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of factual verification datasets with natural inputs. KG denotes knowledge graphs. ChectThat18 has been extended later~\citep{HasanainSEBN19,BarrnCedeo2020OverviewOC,NakovMEBMSAHHBN21}. NELA has been updated by adding more data from more diverse sources~\citep{NorregaardHA19,gruppi2020,gruppi2021}
}
\label{tab:natural}
\vspace{-1em}
\end{table*}
